High-Quality Diversification for Task-Oriented Dialogue Systems

Many task-oriented dialogue systems use deep reinforcement learning (DRL) to learn policies that respond to the user appropriately and complete the tasks successfully. Training DRL agents with diverse dialogue trajectories prepare them well for rare user requests and unseen situations. One effective diversification method is to let the agent interact with a diverse set of learned user models. However, trajectories created by these artificial user models may contain generation errors, which can quickly propagate into the agent's policy. It is thus important to control the quality of the diversification and resist the noise. In this paper, we propose a novel dialogue diversification method for task-oriented dialogue systems trained in simulators. Our method, Intermittent Short Extension Ensemble (I-SEE), constrains the intensity to interact with an ensemble of diverse user models and effectively controls the quality of the diversification. Evaluations on the Multiwoz dataset show that I-SEE successfully boosts the performance of several state-of-the-art DRL dialogue agents.

==> Random.tex <==
%%% This file is created to hold some old text that makes viewing on .tex uneasy and too messy 
%%% These old content might be useful. But unlikely. 
======

%dialogue acts \grace{or a distribution of sequence of actions?} $\{a^u_1, ..., a^u_t ...\}$ over $A^u$. 
%\grace{why you use $u$ here? Aren't they DUME, not base simulator U? For DUME, you used ``'"} \zhiwen{I changed $a^u_t$ to ${a'}^u_t$. As for $A^u$, both $U$ and DUME have the same set of dialogue acts. I have added this point in the problem setup} %We evaluate the diversity as the KL divergence between the distributions of every pair of the user models.

======

%The larger the horizon $H$, the more diverse the resulting trajectory. Setting $H$ too small may cause the policy to be myopic as actions take time to show effects; whereas setting it too large may result in accumulation of errors. We propose to use a moderately small $H=5$ and report an analysis in the experiment section. 


%our method generates parts of a dialogue with the learnt user policies and the other parts are still generated with the user simulator. 
% our method generates parts of the dialogue with the learnt user policies while, the remaining dialogue is still generated using the user simulator.
% Moreover, the learnt user policies only generate trajectories of a short horizon, avoiding the accumulation of errors.


========


% \grace{Is this section mainly talking about using supervised IL to learn a base parametric user model? You should write the math in the way that show it is supervised parametric learning. You should use syntex from ESML textbook chapters 2 and 3. Remember, it is just regression or variations of it} 

% \grace{shouldn't you start the subsection with ``we propose to ...the part in this section's scope ..." ? You need to start with ``what" the method this subsection presents is, instead of jumping into detailed steps. Usually, the beginning sentences for subsections can be extracted (it means they repeat) from earlier overview sections, if you are following normal English writing order. Each paragraph should also have 1 clear theme in that paragraph. And the first sentence in the paragraph should be the overview of the paragraph. }

% \grace{ I think all of the following paragraphs are missing their needed first sentences. The first sentences are simply missing from their positions. Please add them back. And based on the first sentence, introduce more inner structures, such as numbering, listing, ..., in each paragraph. Must pay extra attention in your writing's ordering issue. } 

% \grace{these paragraphs also look out of order among themselves.}


% \grace{this para needs change} We use an ensemble of user models to generate simulations. We train this ensemble with behavior cloning \cite{DBLP:conf/ijcai/TorabiWS18} from the real trajectories. The resulting user models share the same architecture but with different initialization, generating diverse world (user) models. 


=====

% We propose to improve dialogue agent's policy by learning the policy from an ensemble of diverse user models. First, we learn a single user model from the base user model $M_0$ by deep imitation learning. Then, we diversify the neural network's initialization to produce a set of diversified user models. 

%Within the ensemble, we initialize each individual user model differently. Each user model learns to mimic the behavior of the base simulator using behavior cloning  \cite{DBLP:conf/ijcai/TorabiWS18}. The user model ensemble helps generate diverse simulated trajectories. 


========


When using DUME in MFDRL, the model-free method effectively turns into model-based. When using DUME in MBDRL, DUME can replace the single environmenl model to generate more diversified trajectories. 

======
%\grace{why you need to start from $k$? Can you define it as --- $\tau  = [\mathscr{T}_1, ...,  \mathscr{T}_{k}, ... ,\mathscr{T}_{T}]$? Or just $\tau  = [\mathscr{T}_1, ...,  \mathscr{T}_{t}, ... ,\mathscr{T}_{T}]$? }  \zhiwen{No, a branching trajectory would start halfway}

=======

DUME can be used to produce more diverse training trajectories. When using DUME in MFDRL, the model-free method effectively turns into model-based. When using DUME in MBDRL, DUME can replace the single environmental model to generate more diversified trajectories. 


=======

 %\grace{Grace--change here}\grace{add how U will be used differently for MF and for MB. } In both model-free and model-based settings, $M_0$ is treated as part of the environment. 
 
 ======

% \zhiwen{We intermittently switch to interact with DUME and generate trajectories of a short horizon, controlling the diversity of training trajectories in a more sophisticated way.}


=======

Simulator and RL are closely related. Performance of the agent's policy learning largely depends on the quality of the simulator it runs in. 

=======

\begin{scriptsize}
\begin{verbatim} 
User: Hi! I would like to book hotel Leverton House.
System: Leverton House is a cheap hotel.
User: What is the post of Leverton House?
System: Post of Leverton House is cb58rs.
User: What is the type of the hotel?
System: It is a guesthouse.
User: Where is it located?
System: Leverton House is located at 732-
        734 new market road.
User: What is the hotel phone number?
System: You can call the hotel at 01223292094.
User: In which area of the city is this hotel located?
System: There are many attractions in the centre 
        of the city. [***fail***]
User: Ok, bye!
System: Goodbye!
\end{verbatim}
\end{scriptsize}

\begin{scriptsize}
\begin{verbatim} 
User: Hi! I would like to book hotel Leverton House.
System: Hotel Leverton House is located on the east 
        side of the city.
User: What is the post of the hotel?
System: The post of hotel Leverton House is cb58rs.
... 
System: ... Shall I go ahead and book it?
User: Ok! I am not sure about the duration of stay 
      or the number of people staying.
System: Booking confirmed. Anything else?
User: I would also like to book a train from Peterbor
      -ough to Cambridge arriving this Sunday at 15:15.
System: Found a train arriving at 8:38. [***fail***]
User: I want the one arriving at 15:15.
System: Found a train arriving at 6:09. [***fail***]
User: Ok, Bye!
System: Have a good day!
\end{verbatim} 
\end{scriptsize}

\begin{scriptsize}
\begin{verbatim} 
User: Hi! I would like to book hotel Leverton House.
System: Are you interested in booking hotel Leverton
      House on the east side?
User: Where is it exactly located? What is the post, 
      phone and type of the hotel?
System: ... Would you like to go ahead and book it?
User: Ok, Not sure on the duration of stay or number 
      of people as of now.
System: Booking confirmed.
User: I would also like to book a train from Peter-
      borough to Cambridge arriving at 15:15 on Sunday.
System: Would you like to go ahead and book tickets 
      on TR7721? [***correct train***]
User: Ok. Not sure on the number of people.
System: One ticket booked. [***success***]
User: Great! Thanks!
System: Have a good day! 
\end{verbatim} 
\end{scriptsize}

====

\begin{comment}
\begin{lstlisting} 
|\hl{User: Hi! I would like to book hotel Leverton House.}|
|\hl{System: Are you interested in booking hotel Leverton}|
       |\hl{House on the east side?}|
|\hl{User: Where is it exactly located? What is the post,}| 
       |\hl{phone and type of the hotel?}|
|\hl{System: ... Would you like to go ahead and book it?}|
User: Ok, Not sure on the duration of stay or number 
      of people as of now.
System: Booking confirmed.
User: I would also like to book a train from Peterborough
      to Cambridge arriving at 15:15 on Sunday.
System: Would you like to go ahead and book tickets 
      on TR7721? [***correct train***]
User: Ok. Not sure on the number of people.
System: One ticket booked. [***success***]
User: Great! Thanks!
System: Have a good day! 
\end{lstlisting} 
\end{comment}

=======
% Using diverse dialogue trajectories to train task-based dialogue systems can avoid banal  conversations and wrong answers to rare questions.  It is done by automated diversification methods that simulate artificial and diverse trajectories.  These artificial trajectories, however, unavoidably contain generation errors and these errors can  quickly accumulate and propagate in the dialogue systems' learning process.  While it is necessary to make the training data more diverse, it is equally important to keep the training data valid and resistant to unnecessary noise.
%Model-based deep reinforcement learning (MBDRL) enables diversifying the training data by generating simulated trajectories. 


=========


% Selected from a base ensemble of diverse artificial trajectories, we add short segments of the trajectories to real trajectories \grace{what do you mean real trajectory?} every a few time steps. 

% \grace{Please do edit the following two sentences to practice your English and find out what is really wrong. Otherwise, it is too much editing work for me if I must change every single sentence and wording. It is just too much. }

  
% % \grace{could not understand:} I-SEE samples a set of intermediate states from real dialogue trajectories as the starting points of simulation \grace{who are the starting points? whose starting points? Is starting point the correct word? Because they mean number 1. What is 1 about???? The English here is so confusing. Can you tell it yourself? }. Then \grace{Do not use Then. You can use second if needed} it simulates additional branches \grace{what is branches?} of dialogues by having the system \grace{system == I-SEE? What system?} to interact with an ensemble of trained user models for a short horizon 

=====

%Our method learns a set of different environment models, which in turn produce diversified training trajectories. Other MBDRL methods include the following. 
======

Domain randomization directly sets parameters of the environment either randomly \cite{DBLP:conf/iros/TobinFRSZA17} or guided \cite{DBLP:conf/iclr/RuizSC19}. Trajectory synthesis, e.g., hindsight experience replay ~\cite{DBLP:conf/nips/AndrychowiczCRS17,DBLP:conf/aaai/LuZC19},  directly creates new training trajectories by mixing  segments from different existing trajectories. 


========

\noindent {\bf RL-based conversational agents} can be grouped into model-free and model-based methods. {\it Model-Free DRL (MFDRL)} agents take a pre-built environment/simulator as it is and learn policies through directly interacting with it. Various MFDRL algorithms have been proposed for dialogue systems, including deep Q-network (DQN)~\cite{DBLP:conf/ijcnlp/LiCLGC17}, policy-based method~\cite{DBLP:conf/acl/DhingraLLGCAD17}, actor-critic methods~\cite{DBLP:conf/ijcnlp/LiCLGC17} and methods to improve exploration~\cite{DBLP:conf/aaai/LiptonLG00D18,DBLP:conf/emnlp/SuLGLC18,DBLP:conf/emnlp/WuTG20}. It is difficult for MFDRL agent to diversify  training experiences since its environment is fixed. 
======
Deep Dyna-Q (DDQ) \cite{DBLP:conf/acl/GaoWPLL18} is an MBDRL method built upon the classic Dyna architecture~\cite{DBLP:books/lib/SuttonB98}. When DDQ's policy learner interacts with its learned user model, it produces a complete trajectory from the beginning to the end. However, it gives no control over the quality of the newly generated training trajectories. Follow-up work has been proposed to improve the quality of model-generated trajectories. D3Q \cite{DBLP:conf/emnlp/SuLGLC18} uses generative adversarial networks (GAN) to minimize the difference between the model-generated trajectories and the real trajectories from the original built-in user simulator, with the assumption that built-in user simulator is the gold standard. Likewise, ADC \cite{DBLP:conf/emnlp/WuTG20} uses double critics to mitigate the impact of poorly-generated trajectories and stabilize the agent's performance. 

======


Recently,  {\it model-Based DRL (MBDRL)} agents has become quite popular for its inclusion of a model learning module in is design. It allows flexibility in altering the expert environment. MBDRL uses two concurrent learning modules, model learning and policy learning. Model learning employs supervised learning to learn a model $M$ from the expert environment or real human-generated logs. Policy learning then learns  indirectly learn from the model $M$. MBDRL was originally proposed in robotics and control to speed up policy learning by learning an environmental model. Its use in conversational agents is like inserting a middle layer between the original simulator and the policy learner. This middle layer acts as derived simulators. 

=======

%\cite{DBLP:conf/aaai/LiptonLG00D18} improve the exploration of DQN via  Thompson sampling and learn the optimal policy faster. 
%In those algorithms, the agent only communicates with the user simulator

======

 A dialogue agent's  environment consists of a knowledge base and a user simulator. Since the knowledge base usually remains unchanged, most research in model learning refers to learning the user model. 
 
 =====

% The environment of a task-oriented dialogue system consists of two parts, one is the user, while the other is the database. The system agent converses with the user, and queries the database to complete the task. Our method specifically models the policy of the user.


======

%The resulting trajectories enhance the diversity of training data and improve the robustness of the learned policy.


======

The last idea is to diversify the agent's learning experiences by letting it interact with a diverse set of generative user simulators. It is developed as Model-based deep reinforcement learning (DRL) methods and involves little manual configuration~ \cite{DBLP:conf/nips/ChuaCML18,DBLP:conf/nips/JannerFZL19}. 
Model-based DRL methods alternate between learning an environment (user) model (from the expert simulator) and learning a policy from the environment. In our context, the environment (user) model can be thought of simulators. It is a dynamic model that is updated to fit the trajectories that the policy learner collect so far; the policy then is optimized to maximize the long-term rewards within the environment model.  

======

%Without any control, the diversified trajectories generated by the ensemble can largely deviate from what is in a real conversation and become noise. 
%While aiming for more diverse training experiences, it is equally important to keep the experiences legitimate and resistant to unnecessary noise. 


% In this paper, we propose a novel high-quality simulated data diversification method, Intermittent Short Extension Ensemble (I-SEE), that diversifies training trajectories by branching from real dialogue trajectories only every a few steps and only with short artificial trajectories. 

=====

%Diversification is used in simulator-trained CA agents. \grace{the various ways of diversification of dialogue simulations.} 
%Increasing dialogue diversity has been a long-lasting interest. 

======

%Many agents use deep reinforcement learning (DRL) to learn good policies that respond appropriately in a dialogue and succeed in completing the task. Both model-free (MFDRL)~\cite{DBLP:journals/corr/SchulmanWDRK17,DBLP:conf/acl/TakanobuLH20} and model-based DRL (MBDRL) approaches~\cite{DBLP:conf/acl/GaoWPLL18} have been proposed. 

=======

%\citeauthor{DBLP:conf/acl/CampagnaFML20} augmented dialogue data using domain-independent transition rules and domain-specific ontology~\cite{DBLP:conf/acl/CampagnaFML20}. 
%\citeauthor{DBLP:conf/emnlp/NiuB19} synthesized more diverse dialogue trajectories by choosing semantic-preserving language perturbations via reinforcement learning (RL)~\cite{DBLP:conf/emnlp/NiuB19}. 

======

% \grace{Why trajectory is important here? Aren't they only useful for Monte Carlor RL methods? Why they are also useful for DQN, as you used in the evaluation? You need to explain trajectory exactly early in the paper and how it is used}
%Those routine dialogue acts generate trajectories of fixed patterns. Training the system solely on those routine dialogue trajectories does not prepare the system for handling long-tail ones after it is deployed in the real world. 
%As a consequence, dialogue systems trained using rule-based user simulators perform poorly during testing when a real human user spontaneously takes an unusual step in the dialogue or makes an unseen request.
%In the real world, some human users may take an unconventional dialogue act during the interaction, generating long-tail trajectories that are rarely seen in simulators \zhiwen{user simulator $->$ simulator}. System agents that trained on common trajectories \zhiwen{more concrete concept in dialogue scenarios} may not perform well on those long-tail ones. 
%The insufficient exploration in trajectory space does not prepare the system agent well for handling the conversations in the real world. 



=====
%This idea can be extended to MFDRL too, with diverse environment models built to help produce diverse training trajectories.
% This idea can be extended to MFDRL too. Interacting with a diverse set of trained user models changes them into model-based methods and produces diversified training trajectories. 


=======
% \grace{I think letter U confuses with the little u in $s_t^u$, does it? Are they the same thing and should all be u? Otherwise, I suggest we replace the big U with another letter throughout the paper.} \zhiwen{I use $s_t^u$ because this is the state on the user side. It is the same for the base simulator and trainable user models. I agree it is confusing that ppl may only associate it with the base simulator. How about $M_0$ for the base simulator and $M_{\phi_i}$ for the trainable user models?} \grace{OK. please do a universal update for it.} 

===== 
The environment for the agent consists of the user and the knowledge base. But since the knowledge base remains unchanged, in this paper the model (environment) refers only to the user model, which learns patterns and behaviours from human users, and works as a simulator to provide feedback to and converse with the dialogue agent. 

======
increase the diversity of dialogue data with reinforcement learning. 

Their action is data augmentation operations, such as paraphrasing or purposely introducing grammatical errors,  while the reward is the performance of the dialogue system trained on diversified data. 

====== 
%In practice, it can be achieved by changing the parameters of the simulator which the agent interacts with. The changing direction of those parameters can be uniformly random \cite{DBLP:conf/iros/TobinFRSZA17} or guided to improve the agent's performance \cite{DBLP:conf/iclr/RuizSC19}. 

=========

%new trajectories also faces similar challenges, but we handle them in a different way. Instead of generating replacement for real trajectories, we consider model-based experiences as boosters for the training of dialogue agent. Rather than substituting the real trajectories, our method generates model-based trajectories which stem from real trajectories, probing different outcomes of the same dialogue. The model-based experiences give the dialogue agent another push to  explore more effectively.

%Without any control, the diversified trajectories generated by the ensemble can largely deviate from what is in a real conversation and become noise. 

%As the errors in simulation aggregate, the generated dialogues diverge from the real ones. In DDQ, model-based trajectories function as the replacement of real ones. But, using a large amount of model-based trajectories hampers the performance on the contrary. 


%Our method is a model-based approach. It generates model-based trajectories with learned user models. 



% On one hand, we simulate short trajectories to stop the errors from propagating. On the other hand, we view the simulated trajectories as a forced exploration imposed on the system agent and carefully control the amount of simulated trajectories used for training. By prudently handling the extent of divergence between simulated trajectories and real trajectories, our method trains the system agent better.
 

========
%\zhiwen{DDQ sells their idea for sampling efficiency, not for diversification. And they do not have an ensemble. So I changed some wording in this paragraph.} 


=========
\st{$
\tau  = [\mathscr{T}_k, \mathscr{T}_{k+1}, ... ,\mathscr{T}_{k+T}]$}
\st{ $\forall \mathscr{T}_t', a^u_t = M(s^u_t), t>p$ \\ }
\st{ $\mathscr{T}_{k+p}=\mathscr{T}_p'$}


=====

 % \grace{pls check this para} 
%\grace{And I think the major confusion comes from whether $k,p$ and $t$ are moving indexer, or a fixed marker to mark a specific position. Whether they are relevant position or absolution position in a full trajectory starting from 0. What is the relationship between $t$, $k$, and $k+t$ or $t-k$? } \zhiwen{I think defining the base trajectory as $\tau_0$ makes it much more clear. Now $k$ and $p$ are the starting indices of trajectories. $t$ is a moving pointer.}


===========

\begin{comment}
%% E
Ensemble size $E$ is the number of trainable user policies we build. Fig. \ref{fig:exp_ensemble} presents the training curves of several variants of our approach that starts with different $E$. At the beginning, the addition of trainable user policies help improve the performance. But such a trend turns away as more user policies are added.  While increasing the ensemble size does help improve the diversity of the training trajectories, it also enlarges the discrepancy between the simulated trajectories and the real ones. Moreover, it might also build up the risk that a trainable user policy  becomes corrupted. The ensemble size should be carefully set. Sometimes using a larger ensemble not only increases the computation cost, but also degrade the performance.  
%% h
Diversification horizon $h$ is the maximum number of steps in a simulated trajectory. Fig.  \ref{fig:exp_horizon} depicts the training curves of variants of our approach that executed with different $h$. When we decrease the simulation horizon, the performance of the system agent first increases then decreases. Limiting the simulated trajectory to a shorter length helps stop the aggregation of model errors. But it comes with a side effect that, the system agent may not be able to look far enough and optimize the long-term goals in a dialogue.  It will be interesting to investigate how to preserve the model correctness and optimize the system agent in a long run. 
%% \eta 
The amount of simulated trajectories and real trajectories is controlled by parameter $\eta$. The simulation is executed by an ensemble of $E$ trained user policies. The maximum horizon of a single simulation is $h$.
Diversification ratio $\eta$ defines the ratio between the number of simulated trajectories and that of real trajectories. A higher $\eta$ means more simulated trajectories are generated and then used for training. Fig. \ref{fig:exp_ratio} plots the training curves of several variants of our approach that use different $\eta$. Initially, as $\eta$ increases, I-SEE improves the performance of the system agent. As $\eta$ continues increasing, the performance drops. We consider such changes root in the discrepancies between the simulated trajectories and the real trajectories.  Simulated trajectories enhance the diversity of the training data and push the system agent to investigate alternative solutions for the dialogue. It results in the initial improvement of the performance. However, as the amount of simulated trajectories overwhelms that of the real ones, the difference between those two trajectories begins to hinder the performance. In fact, a higher $\eta$ also means more intermediate states will be possibly used as the starting point for simulations. This experiment shows that intermittent extension might be a more preferable way for simulations. It could better balance the diversity of the training data and the discrepancy between reality and simulation. 

\end{comment}

======== 
\begin{comment}


\begin{table*}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|cccccccc}
    \toprule
        Algorithm &  \#Turns & Impr. & Inform F1 & Impr. & Match & Impr. & Success & Impr. \\
    \midrule
         MADPL & 8.96 & & 76.26 & & 90.98 & & 70.1 &\\
\hline
        PPO     & 9.785 & & 86.45 & & 78.90 & & 77.9 &\\
        PPO+Dvs. & 11.39 & & 80.27 & & 70.55 & & 69.0 & \\
        PPO+I-SEE & {\bf 8.88} & {\bf (-0.905, -2.51)} & {\bf 88.06} & {\bf (+1.61, +7.79)} & {\bf 85.83} & {\bf (+6.93, +15.28)} & {\bf 84.5} & {\bf (+6.6, +15.5)}\\
    \hline
        DQN     & 11.54 & & 87.61 & & {\bf 92.91} & & 74.4 &  \\
        DQN+Dvs. (DDQ)  & 11.78 & & 84.26 & & 82.04 & & 72.1 &\\
        DQN+I-SEE & {\bf 9.83} & {\bf (-1.71, -1.95)} & {\bf 89.58} & {\bf (+1.97, +5.32)} & 92.28 & {\bf (-0.63, +10.24)}& {\bf 85.2} & {\bf (+10.8, +13.1)}\\
    \hline
      GDPL & 7.64 & & \textbf{94.97} & & 83.90 & & 86.5 &\\
      GDPL+Dvs. & 9.98 & & 80.86 & & 81.10 & & 72.8 &  \\
      GDPL+I-SEE & \textbf{7.32} & {\bf (-0.0, +0.0)} & 91.83 & {\bf (-0.0, +0.0)} & \textbf{92.76} & {\bf (-0.0, +0.0)} & \textbf{93.2} & {\bf (-0.0, +0.0)} \\
    \hline 
%      %   DDQ & 9.99 & 91.27 & 92.28 & 91.1\\
%      MADPL & 8.96 & & 76.26 & & 90.98 & & 70.1 &\\
%  %       GDPL & 7.64 & \textbf{94.97} & 83.90 & 86.5\\
%   %     I-SEE (PPO) & \textbf{7.32} & 91.83 & \textbf{92.76} & \textbf{93.2} \\
    %    I-SEE (DQN) & 9.94 & 91.50 & 92.44 & 92.0\\
    \bottomrule
    \end{tabular}
    }
    \caption{Dialogue Effectiveness.} % \grace{for each baseline systems, we compare three variations: baseline itself, baseline+full diversification, baseline+I-SEE. The I-SEE results should be the best within each group.} 
    \grace{order the columns in the same order as what is shown in ``eval metrics'. For \#turns, show its improvements by perc. improved so that the numbers will be positive. And only bold improvements when it is positive}
    \label{tab:exp_main}
\end{table*}
\end{comment}

======

% I-SEE provides the dialogue agent with diverse training trajectories and improves the robustness of the agent.

% Table \ref{tab:exp_main} also shows that the full diversification does not help improve the performance at most time. We believe it is due to the accumulation of model errors as the dialogue continues. Thus, the generated diversified trajectories may largely deviate from the base trajectories, introducing noise into the training data. As a result, the policy of the dialogue agent may be biased and is unable to perform well when being tested on the base simulator. As a contrary, I-SEE balances the diversity and noise in the training data and  generate high quality diversified trajectories. After plugging in the I-SEE, the dialogue agent strikes a better balance between exploration and exploitation and achieves higher performance.  
=============
% We choose representative RL algorithms from different categories, i.e. policy-based method, value-based method and model-based method, as baselines. We plug in I-SEE to check if it helps improve the performance (X+I-SEE). As a comparison, we also implemented a full diversification version (X + Dvs) of our approach which use a trained user model to generate complete dialogue trajectories. 

======


\zhiwen{Can we briefly talk about this in the experiments instead of here? I'm worried putting it here gonna raise questions about why we do not control $b$} \grace{Sure they will ask anyways. It is better to defend it up front before they ask. Please add the reason below. I will see where to put it later.}
In addition, 
\begin{equation}
    \eta \propto H \times b
\end{equation}
where $H$ is the simulation horizon, and $b$ is the number of branches. In our experiments, we choose $\eta$ to control the simulation ratio, because \grace{add reason why $\eta$ not $b$?}  Note that ensemble size $E$ has no impact on $\eta$ or $H$. 


========
%We can repeat this branching operation many times on a given base trajectory. The intensity of branching operations determines the amount of branching trajectories generated. The more branchings, the more branching (derived) trajectories. 

%As the amount of diversified trajectories increases, sooner or later, it would outnumber the amount of base trajectories. %As those branching trajectories becomes the majority in the training data, the agent would be mainly optimized for the branching trajectories and ill perform when it is tested on the base simulator. 

=========
In Figure \ref{fig:conceptual}, we generate five diversified trajectories ($\tau_1, ... , \tau_5$) branching from a base trajectory $\tau_0$.  

=====
It is also  important to reduce the noise introduced unintentionally in this interaction learning process. 

=====
 
 Trajectories generated only with $M_{\phi_i}$  may largely deviate from those generated with the base simulator $U$.
 


========
%\grace{Are the following two paragraphs talking about the same thing? Can you combine and shorten them? Keep the essence. } 
%\grace{is this contextual bandits?} \zhiwen{It is not contextual bandits}


===========


Our method I-SEE provides high-quality diversification for training task-oriented dialogue agents. First, we generate a set of base trajectories by having the agent to interact with the base simulator. Those base trajectories will be used along the following steps. 
They will be used to train the user models (second step). They are the stems where branch trajectories ``grow'' (third step). And they are part of the training data of the agent (fourth step).
  
Second, we train an ensemble of user models with imitation learning \cite{DBLP:conf/ijcai/TorabiWS18}. User models learn to mimic the behavior of the base simulator. Each user model is initialized differently, promoting diverse user behaviors. They form DUME. 

Third,  branching from a base trajectory, we continue the dialogue and generate diversified trajectories by interacting with DUME. 

Fourth, we update the agent's policy with both the base trajectories and simulated ones. With the updated policy, our method goes back to the first step and starts a new cycle. 
As a component in MBDRL, our method is built on top of world (user) modeling, and alternates with policy learning. It can be used in conjunction with any model-free policy learning methods.


======


%Mainstream DRL methods require large samples of training trajectories collected from interacting with the user and the environment. In task-oriented dialogue systems, this sampling process becomes impractical since human-generated feedback is too expensive to get.
========
% Those model-based DRL methods learn the system policy and environment models alternatively.  When learning the environment model, these methods learn a supervised parametric model to best describe the environmental dynamics; When learning the system policy, these methods update the system's policy in the direction that optimizes the long-term expected rewards within the learned environment model. 

% \grace{the following assumes MB is for diversity. It seems not true. How to present it?} \grace{how do other MBDRL methods do diversification? Do they care?}

=========

% \grace{you need to BRIEFLY talk about the NN that you use. Because later on in the next subsection, we need to talk more about it.} 

% \grace{input? output? mapping function (from input to output)?}
%Training a user model is a multi-task learning problem \grace{not any more if you put ending as an action}. 
% The main task of a user model is to choose the most appropriate dialogue acts at the current state. 
% We regard the mapping from $s^u_t$ to $a^u_t$ as a multi-class classification task \grace{no, a sequence of states are your input}. We update the user model by cloning the behaviors from the user simulator. The loss function is shown in Eq. \ref{eq:wm_loss}:

% \grace{change ending to one of the actions and combine the following with Eq. 1 and the paragraph before Eq.1}
% In addition, we also learn the ending states for the dialogue in the user model. Given that a dialogue usually ends when both the user and the agent say ``goodbye" or the user goal is abandoned without being satisfied. We propose to estimate when the dialogue would end by a binary classification. With the same $s^u_t$ as input, user models estimate whether the dialogue ends or not. We update the user model with binary cross-entropy in Eq. \ref{eq:wm_d_loss}. 
% \begin{equation}\label{eq:wm_d_loss}
% \begin{split}
%     L(\phi)  = - \frac{1}{T} & \sum_{t=1}^T d_t \log M_{\phi}(s^u_t)_d + \\
%     & (1-d_t) \log (1 - M_{\phi}(s^u_t)_d)
% \end{split}
% \end{equation}
% where $M_{\phi}(s^u_t)_d$ is the estimated probability of whether the dialogue ends at time step $t$ and $d_t$ is the ground-truth label of whether the ending is $t$. 

% The supervised method used to learn the user model is neural network. We construct an  individual user model as multi-layer perceptron and train it by behavior cloning from the base trajectories.  % \grace{add details, emphasis parameter $\phi$, and your assumptions -- why you break sequence into individual pairs.} 

=================
%Third, we sample a set of intermediate states from real trajectories and branch the dialogue. The system agent interacts with the ensemble of user models for a short period of time, generating simulated trajectories. 


% First, we learn a world (user) model with supervised imitation learning. Interacting with this user produces ``real trajectory"  Second, we diversify the world model with different initialization, which creates an ensemble of diversified artificial user models. Interacting with these diversified user models produces ``artificial trajectories". Third, when the policy learning starts, the agent mainly interact with the real user model, but from time to time,  the agent interacts with the diversified ensemble and branches away from the original real trajectory. The connecting points are uniformly randomly chosen.  
% Fourth, to prevent errors aggregated from long artificial trajectories, we only extend the real trajectories within a short horizon. 



=============
% \grace{It is very important that for each section, you mention what is its input and what is its output. They are not codes but their inputs and outputs would help sections before and after this section to better connect to them. If a section is about a function in your code, then never forget to mention key ingredients -- inputs, outputs, optimization objectives and constraints, methods in the blackbox, and hyper-parameters. Please add them back to each of your sections. } 


=============


%Generating simulated experiences requires building environment models. 
% \grace{this paragraph should be part of the introduction. And it needs to be shorten to only cover the main points. They should be inserted before ``Early user simulators ..." and much shortened. } 
% In a task-oriented dialogue system, the environment for the system agent consists of two parts: the database and the user simulator \grace{too late to appear this definition of user vs. environment. That was why I had so many questions in intro about it. You need to move them before any questions raised}. The database stores static records of task-specific knowledge. For example,  a dialogue system that helps book air tickets is equipped with a database that stores all the flight information. The user simulator takes actions based on previous interaction and pushes forward the conversation.  When modeling the environment, we build user policies that act as the user simulator, but still use the same database. Such a choice has several benefits. On one hand, the system agent uses the same database in training and testing. It is unnecessary to model the database querying process, which introduces additional complexity of modeling the environment and brings in unrealistic or even illegal actions. On the other hand, long-tail trajectories directly result from unusual user actions. Building the user policies would be sufficient to generate simulated dialogues.  


% Figure \ref{fig:system} gives an overview of our system \grace{ours or any model-based DRL dialogue systems? I think it is the latter. Because of this, this figure should be moved to introduction too. After ``...model-based DRL methods. (Janner et al. 2019) ..." }. Our system includes an ensemble of trainable user policies. \grace{is ensemble also novel in this paper? Or only short and intermittent are two novel ideas? Do you have 2 or 3 novel ideas here? I mean for task-oriented dialogue systems?} Each trainable user policy is mimicking the behavior of the user simulator \grace{I dont think this imitation learning part is novel, I think you can just cite another paper who also did it}. \grace{basically the remaining sentences in this paragraph are unclear. It is because it is unclear how many novel ideas you have. This will determine whether and how these sentences should be said. Nonetheless, the following sentences are lack of structure. They have the same type of issue as the first paragraph in this section -- no clear structure and don't know why they appear. They also repeat points that have already been made earlier. } 
% The system agent either interacts with the user simulator or the trainable user policy ensemble. During the interaction, the agent samples the actions based on the dialogue acts of the user and the querying results from the database. The agent's policy is updated with both the real trajectories and the simulated ones. In the remaining part of this section, we will detail how to train user policies and how to update the agent's policy.


===================

% \subsection{Policy Optimization}

% \grace{I am not sure why you only introduce PPO here? I think your method is independent of how policy will be learned. That means, it supports value-based methods too, right? That is why in your experiments, you have DQN and DDQ to compare with, right? Think of what you propose here is a component in data-generation DRL, so your method can be used in combination with any DRL model-free method, right? that is why I have question why you specially talk about PPO here. } 
% We train the system agent on both the real trajectories and simulated trajectories. The diversity-enhanced training trajectories enable the system agent to continuously explore the space of dialogue trajectories. During training, the system agent does not distinguish the real trajectories and simulated trajectories. It is optimized using proximal policy optimization (PPO) \cite{schulman2017proximal}.
% \begin{equation}\label{eq:ppo}
%     \begin{split}
%         L(\theta) = & \mathbb{E}_t[ r_t(\theta)\hat{A}_t, clip(r_t(\theta), 1-\epsilon, 1+\epsilon) \hat{A}_t \\ 
%         & - c (V_\theta(s_t) - V_t^{targ})^2 ]
%     \end{split}
% \end{equation}
% where $\theta$ is the policy parameter. $r_t(\theta)=\frac{\pi(a_t|s_t)}{\pi_{old}(a_t|s_t)}$ denotes the difference in action probabilities before and after the policy update. $\epsilon$ is the clipping ratio. $clip(r_t(\theta), 1-\epsilon, 1+\epsilon)$ clamps $r_t(\theta)$ within the range $[1-\epsilon, 1+\epsilon]$.  $V_{\theta}(s_t)$ is the estimated state value of $s_t$. $\hat{A}_t$ is the advantage function and is calculated as Eq. \ref{eq:adv_defn}
% \begin{equation} \label{eq:adv_defn}
%     \hat{A}_t = \delta_t + (\gamma\lambda) \delta_{t+1} + ... + (\gamma\lambda)^{T-t+1} \delta_{T-1}
% \end{equation}
% where $\delta_t = r_t + \gamma V(s_{t+1}) - V(s_t)$ and $\lambda$ is the generalizing factor for generative advantage estimator \cite{DBLP:journals/corr/SchulmanMLJA15}.


=========
% In a task-oriented dialogue system, the environment for the system agent consists of two parts: the database and the user. The database stores static records of task-specific knowledge. For example, the database of a dialogue system that helps book air tickets stores the flight information. The user usually has a goal in mind before the conversation starts. During the conversation, the user takes actions based on the goal and responses from the system. The database is static while the user dynamically pushes forward the conversation. Instead of modeling the whole environment that includes both the database and the user, we only model the user. Such a choice has several benefits. It reduces the complexity of modeling a complex environment. It also keeps the world model from generating database querying results that are unrealistic or even illegal. 


==========

A natural way to exploit the trained user models is to use them to generate complete dialogues. But such a usage may face unavoidable drawbacks. Model-based DRL algorithms alternate between model learning and policy updating. The system policy is updated with simulated trajectories generated by the model, while the model is trained with trajectories collected with the system policy. In consequences, errors in simulations may degrade the performance of the system policy, while a biased system policy may collect trajectories that further mislead the environment model. Such errors compounded on and on.  Their propagation prevents the continuous improvement of the system policy.   


==========

% Interactive systems, such as search engine and dialogue systems, have become a necessary part of human's daily lives. Those systems are designed to assist human users to complete the tasks in a back-and-forth conversation. Reinforcement learning (RL) is a natural fit for this type of problems because of its interactive and goal-oriented nature. Deep RL algorithms represent the agent's policy with a deep neural network and optimize the policy in a data-driven way. The optimization step requires intensive sampling of the agent's trajectories. In interactive systems, this sampling process is more expensive since humans are involved. As the task complexity increases, it becomes impractical to build the interactive agents with real human users. 

===============

% In this paper, we show that we can overcome this limitation by diversifying the dialogue trajectories. We augment the training trajectory with simulated conversation stem from real ones. As a complementary to the real trajectories, simulated trajectories enhance the diversity of the training data, encourage the exploration the system agent. We train multiple user policies by learning from the user simulator,  then simulate the dialogue by having the system agent to interact with learnt user policies.  Each learnt user policy will show distinct behavior as they are initialized differently. Every simulated dialogue starts from a randomly sampled state in real conversations. Then the system agent interacts with a sampled user policy to extend the conversation. Those simulated dialogue trajectories are like imagined conversations, where the system agent can practice with a virtual user who may proceed the conversation in a different style. Those simulations present the agent with the possibilities of a different future in a conversation. The simulation continues as the real interaction goes on, enabling the system agent to explore different branches of a dialogue. Thus, the system agent is better prepared for handling conversations that rarely shows in the user simulator. After deployment, the system agent perform better on long tail conversation trajectories. 



============

\begin{comment}
% Methods enhancing the diversifying of training dialogue trajectories have been proposed. They are known as the data-generation model-based DRL methods~\cite{DBLP:conf/nips/JannerFZL19}. 
% The system learns its policy through interacting with an ensemble of diversified user models, each of which simulates distinct user behaviors with different initialization. 

%Simulated dialogues, which result from the interactions between the system agent and the trained user policies, enhance the diversity of the training data and encourage the exploration of the system agent.   

% \zhiwen{introduce model-based RL, explain why error propagates}
% Those model-based DRL methods learn the system policy and environment models 
%\grace{I suggest to call user models, instead of user policies throughout the paper.}
% alternatively. 
% When learning the user model, these methods learn a supervised parametric model to best describe the environmental dynamics; When learning the system policy, these methods update the system's policy in the direction that optimize the long-term expected rewards within the learned user model %\grace{user and environment, are they one model or two separate models?}. 
% But such training paradigm have some drawbacks. As the alternative learning steps proceed, learning errors from supervised environment modeling quickly accumulate and propagate. The resulting simulated training trajectories can largely deviate from  any trajectory % that a real human can think of % \grace{give concrete example here.} 
% and become noise in the training data.  
%The imperfect environment model generates transitions that diverge from the real ones.
% As the dialogue unfolds, such kinds of errors aggregate, the simulated trajectories may largely deviate from the real trajectories.
%As the dialogue unfolds, these errors aggregate. 
% While we recognize the necessity to make the training data more diversified, it is equally important to keep the training data valid and resistant to unnecessary noise.  


% In this paper, we propose to use a hybrid type of training trajectories, which are simulated short trajectories intermittently extended from real trajectories. This novel trajectory diversification method is called {\bf Intermittent Short Extension Ensemble (I-SEE)}. When diversifying simulated trajectories by an ensemble of user models, %Each trained user policy may extend the dialogue in a different style. 
% We propose to use a segment from a real dialogue trajectory, and extend it with a short segment generated by simulation. \grace{give concrete example here.} This is to prevent the estimation errors from aggregating. %, while extending the real dialogue towards possibly different directions.  
% \grace{what is about direction??}
% The connecting points of the real trajectory and the simulated trajectory can be are uniformly random. 
%enabling the system agent to investigate possible alternatives at all points during a dialogue.  
% In addition, we only perform such extension at every a few learning steps, to avoid noise built up too quickly. 
% Our method provides controls over the training trajectories' quality while still presents the system agent with more diverse training trajectories. % of high fidelity. 
% Our experiments are conducted over the Multiwoz \cite{budzianowski2018multiwoz} dataset. Compared with the state-of-the-art approaches, our method is highly-effective. It provides high-qualify diversification and achieves better performance. 

\end{comment}


======================


% The main idea of our approach is to diversify the training trajectories with world models. Previous works have been focusing on improving the sample efficiency with world model \cite{peng2018deep}, while we are working towards a different end. Our method generates diverse simulated trajectories that forked from the real ones. The exploration of the system agent is then powered from two different fronts. One is its internal action sampling mechanism, such as $\epsilon$-greedy. The other is the external turbulence imposed by world models, which is our focus. The system agent thus is able to continuously explore in the trajectory space in the training process.

% Our method aims to automatically generate high-quality diverse trajectories to train task-oriented dialogue systems. \grace{the remaining sentences in this paragraph are super unclear. They have no good connections. No overall relations to govern each sentence under one umbrella. Are you talking steps? Then number them. Or, are you presenting a general-specific-general structure? Then do it. Make the structure EXPLICIT. Please rewrite this para. }  We achieve this goal by having the system agent to interact with different environment \grace{user model or environment model??} models. We obtain an ensemble of models by imitation learning from the real environment. Different environment models may respond to the actions of the system agent following different dynamics. The simulation with a set of learnt environment models enhances the diversity of the training experience. 


==> method.tex <==

\section{Proposed Work}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{fig/system.png}
    \caption{System Architecture.} 
    \label{fig:isee_system}
\end{figure}



Our method aims to provide high-quality diversified training trajectories for dialogue agents. We take an approach of model-based DRL (MBDRL). It has two concurrent learning modules, model learning and policy learning. 
The {\it model learning} module can be thought of adding an additional computational layer between the original simulator and the agent. 
Model learning employs supervised learning to learn a transition model $M$ from the original environment and then policy learning interacts with the model $M$ and learns indirectly from the environment. 
We propose to improve dialogue diversity by having the agent interact with an ensemble of diverse user models $\{M_{\phi_*}\}$. To create the ensemble, we (1) use neural network with different initialization to learn them from expert user model $M_0$.  We then (2) intermittently generate short trajectories with DUME and use them in policy learning.
% acquire DUME-generated trajectories intermittently and within a short horizon for policy learning. 
The DUME is obtained via mimicking user behaviors from the expert simulator. 
%We take advantage of the learning discrepancy of the resulting user models. 
%The training trajectories from DUME are only generated  intermittently and within a short horizon. 
Our goal is to reach a balance between data diversity and quality. Figure \ref{fig:isee_system} illustrates  our system architecture. 


% These user models mimic real user behaviors; however they cannot achieve 100\% learning accuracy. On one hand, instead of mitigating the difference between trajectories generated by real user simulator and the the ensembles, we take advantage of the differences to enhance the diversity of training for the agent's policy learning. On the other hand, we incorporate these artificial trajectories with great caution. Aware of the unavoidable learning errors innate in them, we propose a novel method to only use artificial data intermittently, and only use a short horizon of them. Our goal is to reach a balance between data diversity and data quality. 

%The learned user model may behave differently from the the simulator which uses hand-crafted rules. Such difference provides the system with the possibility of a different interaction process. It forces the system agent to explore a different approach to complete the task. The simulated trajectories then serve as complementary to the real ones. They prepare the system agent for handling long-tail trajectories after deployment. 


%\subsection{Constructing a Diverse Set of User Models}
% 1. Why only models user action
% 2. Why only fork short trajectories
% 3. Why ensemble

% \grace{Is this section mainly talking about using supervised IL to learn a base parametric user model? You should write the math in the way that show it is supervised parametric learning. You should use syntex from ESML textbook chapters 2 and 3. Remember, it is just regression or variations of it} 

% \grace{shouldn't you start the subsection with ``we propose to ...the part in this section's scope ..." ? You need to start with ``what" the method this subsection presents is, instead of jumping into detailed steps. Usually, the beginning sentences for subsections can be extracted (it means they repeat) from earlier overview sections, if you are following normal English writing order. Each paragraph should also have 1 clear theme in that paragraph. And the first sentence in the paragraph should be the overview of the paragraph. }

% \grace{ I think all of the following paragraphs are missing their needed first sentences. The first sentences are simply missing from their positions. Please add them back. And based on the first sentence, introduce more inner structures, such as numbering, listing, ..., in each paragraph. Must pay extra attention in your writing's ordering issue. } 

% \grace{these paragraphs also look out of order among themselves.}


% \grace{this para needs change} We use an ensemble of user models to generate simulations. We train this ensemble with behavior cloning \cite{DBLP:conf/ijcai/TorabiWS18} from the real trajectories. The resulting user models share the same architecture but with different initialization, generating diverse world (user) models. 



% We propose to improve dialogue agent's policy by learning the policy from an ensemble of diverse user models. First, we learn a single user model from the base user model $M_0$ by deep imitation learning. Then, we diversify the neural network's initialization to produce a set of diversified user models. 

%Within the ensemble, we initialize each individual user model differently. Each user model learns to mimic the behavior of the base simulator using behavior cloning  \cite{DBLP:conf/ijcai/TorabiWS18}. The user model ensemble helps generate diverse simulated trajectories. 

\subsection {Diversified User Model Ensemble (DUME)}

We propose to build a diversified user model ensemble to produce more diverse training trajectories. The ensemble, DUME,  contains a set of $E$ number of user models $M_{\phi_1}, M_{\phi_2}, ... , M_{\phi_E}$. Each user model ($M_{\phi_*}$) is trainable and learns a parametric mapping from $s^u_t$ to ${a'}^u_t$ with parameter $\phi_*$ and mimics the behavior of the expert simulator $M_0$. 

We aim to learn a sequential decision-making function that maps $(s^u_1, s^u_2, ..., s^u_t...)$ to $ (a^u_1, a^u_2, ..., a^u_t, ...)$. The training inputs are from expert trajectories, which includes a sequence of user state and user action pairs $\langle s^u_t, a^u_t\rangle$.  User state at the $t^{th}$ dialogue turn is 
\begin{equation} \label{eq:user_state_defn}
    s^u_t = (G, \bigcup_{t'=1}^{t-1} a^s_{t'})
\end{equation}
where $G$ is the user goal, including constraints and requests. $\bigcup_{t'=1}^{t-1} a^s_{t'}$ is history of dialogue agent actions. 
The user action $a^u_t$ is defined as 
\begin{equation} 
a^u_t=(a^u_{t, 1}, a^u_{t, 2}, ... , a^u_{t, |A^u|})
\end{equation}
where $a^u_{t, i}$ are binary variables indicating whether the $i^{th}$ dialogue act is active at dialogue turn $t$. $A^u$ are the available user dialogue acts. Note that a single user action can have multiple dialogue acts. E.g.,  informing the destination and arrival time at the same time when booking a train ticket. Ending of a dialogue is a special dialogue act. 

The user model is learned by behavior cloning~\cite{DBLP:conf/ijcai/TorabiWS18}.  
We break the training input sequence $\tau_0$ into individual state-action pairs and formulate the learning as to choose the right dialogue acts at a given state, i.e. a mapping from $s^u_t$ to $a^u_t$. This simplification is done because a user may take a varied number of dialogue acts at each turn, modeling state-action pairs allows the flexibility. The optimization is done by minimizing the loss function $L(\phi)$:
\begin{equation}\label{eq:wm_loss}
\begin{split}
    L(\phi) = - \frac{1}{|A^u|} \frac{1}{T} &  \sum_{t=1}^T \sum_{i=1}^{|A^u|}  a_{t, i} \log M_{\phi}(s_t^u)_i + \\
                                    & (1-a_{t,i}) \log (1 -  M_{\phi}(s_t^u)_i  )
\end{split}
\end{equation}
where $\phi$ is the model parameter vector, $a_{t,i}$ is the ground truth indicator of whether the $i^{th}$ dialog act is taken at $t$, and $M_\phi(s_t^u)_i$ estimates the probability of the $i^{th}$ dialog act being chosen by the user model at $t$ given $s^u_t$. The learning is done by a multi-layer perceptron neural network parameterized by $\phi$. 

%individual dialogue act  we let the user model predict whether each individual dialogue act should be taken.


% Since $s^u_t$ already contains part of the historical sequential information ($\bigcup_{t'=1}^{t-1} a^s_{t'}$), we formulate this task as learning to choose the right dialogue acts at any given state, i.e. a mapping from $s^u_t$ to $a^u_t$. Such a formulation also eases the implementation.  

% We break the trajectory into a set state-action pairs and use them to update the user model.
% The number of active dialogue acts in a state may vary per time step. Thus, at every time step, we let the user model predict whether each individual dialogue act should be taken. 


Note that this user modeling can be done using much more sophisticated methods. E.g. we can use more advanced network and/or incorporate more information when defining user states. However, they are beyond the scope of this paper. Our user models are sufficient to support our investigation in exploiting them to improve diversification.  

% \subsection{Generate Diversified Simulators} 

% The neural network' architecture is learned from the base user model by behavior cloning (Section 3.3.1).  % \grace{more details; be mathematical. your output should be a set of user models}

% \grace{also add how it can be used to generate diverse user models? what do you think about the learning error here? good or bad? I remember you said you think it is an advantage. So elaborate. } 

DUME diversifies user models by initializing them with different seeds.  Their neural networks share the same architecture but having different initial parameters $\phi_j$. Our experiments (Section 5.4) show that when $E$ increases, the diversity in DUME dramatically increases. 


%When interacting with the dialogue agent, DUME creates more diverse trajectories for policy learning. 

% The learned user model can be diversified by creating an ensemble of neural networks of the same architecture but with different initial parameters $\phi$. Each user model is trained with behavior cloning using base trajectories. After the training, we obtain a set of $E$ number of user models, $M_{\phi_1}, M_{\phi_2}, ... , M_{\phi_E}$, each with unique parameters $\phi_i$. When being queried by the policy learner,  this diverse user model ensemble can create more diverse trajectories for policy learning. 

% \grace{is there any way mathematically to measure the differences between any two models? How to show this error? KL divergence or cosine sim? I think will be something about $|\phi_i-\phi_j|$I think we can use it in exp to show degree of diversification}

%Our method exploits the discrepancy between the user model and the base simulator. Such a discrepancy always exists and different user models may bias in different ways. By building an ensemble of user models, our method simulates users of different types.  The agent has more chances to be exposed to more types of users, making it ready for handling long-tail trajectories.  

%\subsection{Control the Quality of Diversification}

\subsection{Policy Learning with Branching} 

\begin{algorithm}[t]
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{User model $M$, \\
        system agent policy $\pi$, \\ starting user state $s^u_0$,\\ maximum trajectory length $T$}
\Output{
% Dialogue trajectory dataset $D_{sys}$,\\ User action dataset $D_{user}$
Dialogue trajectory dataset $D$\;
}
% $D_{sys}, D_{user}=\varnothing, \varnothing$\;
$D = \varnothing$\;
initialize the user state to $s^u_0$\;
\For{$T$ time steps}{
        The user model observes the state $s^u_t$ and takes action $a^u_t=M^i(s^u_t)$\;
        % The user takes action $a^u_t=M^i(s^u_t)$\;
        The agent observes the state $s^s_t$ and takes action $a^s_t = \pi(s^s_t)$\; 
        % The agent takes action $a^s_t = \pi(s^s_t)$\;
        The agent receives reward $r_t$\;
        Store $\langle s^s_t, a^s_t, r_t, s^u_t, a^u_t \rangle$ in $D$\;
        % Store $\langle s^s_t, a^s_t, r_t\rangle$ in $D_{sys}$\;
        % Store $\langle s^u_t, a^u_t, d_t\rangle$ in $D_{user}$\;
        \If{the user decides to end the dialogue in $a^u_t$}{
            break\;
        }
    }
%\Return $D_{sys}, D_{user}$\;
\Return $D$
\caption{Trajectory Generation} \label{algo:traj_gen}
\end{algorithm}


To diversify the policy learning, a natural solution is to interact with user models in DUME and generate a set of diversified trajectories. When generating trajectory, the policy learner, i.e. the agent, interacts with a user model, which is either the base user model $M_0$ or a diversified user model $M_{\phi_j}$. Their interaction works as follows. The user starts the dialogue with a task goal. The agent performs an action based on its current policy $\pi$ and receives rewards and next state from the user model. The user's action are decided by the user  model too. The agent responds again based on $\pi$ and the trajectory continues until the dialogue ends. Algorithm \ref{algo:traj_gen} details this trajectory generation process. The agent collects this training trajectory, together with many other trajectories simulated likewise, to refine its policy to a better policy.

%Note that trajectories can be generated from either a base user model or a diversified user model. 
% This process works the same for the agent interacting with $M_0$ or $M_{\phi_i}$.


\begin{algorithm}[t] 
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{User model ensemble size $E$\\ diversification horizon $H$\\ diversification ratio $\eta$}
\Output{System policy $\pi$}
initialize an ensemble of $E$ user models\;
initialize the dialogue agent policy $\pi$\;
\While{ the dialogue policy does not converge}{
 % $D_{real}, D_{u} = \varnothing, \varnothing $\;
 $D_{exp}, D_{dvs} = \varnothing, \varnothing$ \;
  \For{every episode}{
  initialize the base user simulator $M_0$\;
  observe the initial user state $s^u_0$\;
  $D_{exp}=$TrajectoryGeneration$(M_0, \pi, s^u_0, \infty)$\;
  }
  % $D_{sim} = \varnothing $\;
  \While{$|D_{dvs}| < \eta |D_{exp}|$}{
    sample a user model $M_{\phi_j}$ from the ensemble\;
    sample a state $s^u_t$ from $D_{base}$ as the start state\;
    \begin{tabular}{l}
         $D_{dvs}= D_{dvs} \bigcup$ \\
         TrajectoryGeneration$(M_{\phi_j},  \pi, s^u_t, H)$\; \\
    \end{tabular}
  }
  Update the agent policy $\pi$ with $D_{base} \bigcup D_{dvs}$ \; % Eq. \ref{eq:ppo}\;
  Update the user model ensemble with $D_{base}$ using Eq. \ref{eq:wm_loss}\;
}
\caption{Intermittent Short Extension Ensemble (I-SEE)} \label{algo:i-see}
\end{algorithm}

A {\bf diversified trajectory segment $\tau_p'^{p+H}$}. It is a trajectory that records the interaction between $M_{\phi_*}$ and the agent. It extends base trajectory $\tau_0$ from a branching step $p$ and runs from $p+1$ onward. It is denoted as: 
\[
\tau_p'^{p+H} = [\mathscr{T}_p, \mathscr{T}_{p+1}', ... ,\mathscr{T}_{p+H}'], 
\]
where $p$ is the branching step and $p>0$.
Note that the first interaction tuple in $\tau_p'$ is copied from the $p^{th}$ turn in $\tau_0$:  $\mathscr{T}_p'= \mathscr{T}_{p}$. $H$ is $\tau_p'$'s horizon. 


%We may produce as many as full diversified trajectories  using random $M_{\phi_i}$ in DUME. These trajectories are used by the agent to learn its policy. 
One would imagine that the more diversified trajectories used in training, the more robust the policy would be. An intuitive idea is to interact with the diversified user models $M_{\phi_*}$ from beginning to the end, without using $M_0$ at all. 
DDQ \cite{DBLP:conf/acl/GaoWPLL18} indeed exploits this design. However, a dialogue trajectory completely generated by $M_{\phi_*}$ suffers from accumulation of generation errors because they may  deviate too much from what a real dialogue looks like. %Errors accumulate too much in the policy as the policy learner queries the user model for a long horizon. 


In this paper, we propose to generate trajectories from mixed sources. The trajectories are generated from both the expert user simulator $M_0$ and DUME. 
First, we generate a full expert trajectory $\tau_0^{T}$=$[\mathscr{T}_0 ..., \mathscr{T}_{T}]$ and store all its tuples.  Second, we pick a branching tuple $\mathscr{T}_p$ from $\tau_0^{T}$ as the branching point $p$. Third, from $p$ onward, the trajectory is generated with a diversified user model $M_{\phi_*}$, which would take an action ${a'}^u_p$ different from the base action $a^u_p$ and the agent would also land in a different state ${s'}^s_{p+1}=P(s^s_p, a^s_p, {a'}^u_p)$. Such interaction with $M_{\phi_*}$ continues with $H$ steps, resulting a diversified trajectory $\tau_p'^H = [\mathscr{T}_p', \mathscr{T}_{p+1}', ... ,\mathscr{T}_{p+H}']$. Note that we re-use the stored base tuple $\mathscr{T}_p$ and $\mathscr{T}_p'=\mathscr{T}_p$. The  full trajectory with diversification is $[\mathscr{T}_0, ..., \mathscr{T}_p, \mathscr{T}_{p+1}', ...,\mathscr{T}_{p+H}']$.  


 
 


 
 
% However, since no learned user policy performs perfectly, errors will  accumulate over time. Dialogues generated with the learnt user policy may largely deviate from those generated with the real user or the user simulator.  As a consequence, the system agent trained with such simulated trajectories may not perform well. 


%Our method generates dialogue trajectories that branch to a different direction at a point and continues with a branching diversified trajectory. 

%\grace{The paper sometimes use $h$ sometimes uses $H$ for simulation horizon; pls change all to be consistent. It appears in section 4 and 5. In text, algorithm, experimental results, Figure 5, and formulas.}

%In this paper, we propose to control the quality of diversification by using DUME more conservatively. 


{\bf Branching Horizon.} The hyper-parameter $H$ is the simulation horizon that controls how far a trajectory is generated from DUME. Our experiments show that using a moderately small $H=5$ is preferable. Figure \ref{fig:conceptual} illustrates this idea conceptually. 


%The larger the horizon $H$, the more diverse the resulting trajectory. Setting $H$ too small may cause the policy to be myopic as actions take time to show effects; whereas setting it too large may result in accumulation of errors. We propose to use a moderately small $H=5$ and report an analysis in the experiment section. 


%our method generates parts of a dialogue with the learnt user policies and the other parts are still generated with the user simulator. 
% our method generates parts of the dialogue with the learnt user policies while, the remaining dialogue is still generated using the user simulator.
% Moreover, the learnt user policies only generate trajectories of a short horizon, avoiding the accumulation of errors.


{\bf Branching Frequency.} Another factor that determines the degree of diversification is the intensity of branchings. We propose to control the amount of diversified  trajectories branching out from the expert trajectory. Instead of branching at every single step, our method only intermittently forks a diversified trajectory. 
It is done by setting a diversification ratio $\eta$ between the times the agent interacting with the expert simulator $M_0$ and with DUME. The ratio $\eta$ is calculated as:  
\begin{equation}
    \eta = \frac{count(\mathscr{T}'_i, \forall i \in D_{dvs}) }{count(\mathscr{T}_j, \forall j \in D_{base})}
\end{equation}
where $\mathscr{T}'_i$ is a diversified interaction tuple stored in $D_{dvs}$ and $\mathscr{T}_j$ is an interaction tuple stored in $D_{exp}$. $D_{exp}$ and $D_{dvs}$ are collections of individual interaction tuples obtained as Lines 4-14 in Algo.~ \ref{algo:i-see}. A larger $\eta$ means more diversified the agent's learning is.
Algo.~\ref{algo:i-see} shows the entire I-SEE algorithm.


%We record every time step in the dialogue as a tuple $\langle s^s_t, a^s_t, r_t, s^u_t, a^u_t \rangle$, where $s^s_t, a^s_t$ are the state and action of the system, $s^u_t, a^u_t$ are the state and action of the user (either the base simulator or a diversified user model), and $r_t$ is the reward the agent receives. 


% \grace{the following para seems misplaced.} 
% To further enhance the diversity, we introduce an ensemble of $E$ user models. We sample a user model when a simulation begins and continue using it until that simulated trajectory is completely generated. 

% A single learnt user policy is unlikely to perform perfectly. Thus, we propose to use an ensemble of learnt user policies to reduce the bias of a single one. Each simulated trajectory is generated with a learnt user policy sampled from the ensemble. In practice, we first generate complete real trajectories with the user simulator. Then, we randomly sample states from the real trajectories as starting states for simulation. At every starting state, we first sample a learnt user policy, then use that policy to generate simulated trajectories. 



% \subsection{Algorithm}

% We present our algorithm, intermittent short extension ensemble (I-SEE), in Algo. \ref{algo:i-see}. I-SEE starts by interacting with the user simulator to collect real trajectories. After that, I-SEE samples a set of branching points, and generate short extensions of the dialogue. Those branches represent alternative action choices at given states. The system agent is presented with dialogue states that it rarely encounters when it only interacts with the user simulator. Short simulation trajectories prevents the errors from aggregation, ensuring the learned user model still behaves reasonably. Intermittent extensions strike a balance between the diversity and noise level of the training data. In all, I-SEE generates high-quality simulations that diversify the training trajectories. 


% \subsection{Simulated Dialogue Generation}
% It has been a hard task for model-based RL algorithms to mitigate the difference between the real trajectories and the simulated ones.  The difficulty comes from two reasons. On the one hand, it is virtually impossible to build an environment model that mimics the real environment with 100\% correctness.  On the other hard, even if a environment model perfectly predicts the environment dynamics,  there still exists some discrepancy between the training environment and the deployment environment. This discrepancy is also referred to as the reality gap in the literature, a factor that has to be considered when the agent is trained on simulator but deployed in the real world. As the dimension of state/action space grows, it becomes harder and harder to model the environment accurately and the reality gap is more and more increased. 


% \grace{I think if you provide a good math definition of a trajectory earlier, you can now show a formula of ``extension" by using segment a + segment b. You can also use formulas to show for every few steps, you do the extension and how short and far it will be extended. }





==> related_work.tex <==
\section{Related Work - \grace{Hrishikesh, could you please work on related work ? thanks}} 


\grace{this section is out of order. Please write in the order of areas A, B and C; or follow the format and order of related work section of SIGIR 2019 best paper.} 
\grace{suggest to use subsections}
\grace{I also think you can cite my ACL 2020 paper and some of its references. It is about diversity and dialogues.} 

\grace{Past work has improved model diversity with innovation on model architectures and decoding strategies (Li et al., 2016a; Baheti et al., 2018; Li et al., 2017; Shao et al., 2017; Cao and Clark, 2017; Serban et al., 2017; Zhao et al., 2017). We ..."
in
http://infosense.cs.georgetown.edu/publication/117.pdf}

Our method is a model-based approach. It generates simulated trajectories with learnt user policies. Prior to our work, Deep Dyna Q (DDQ) \cite{DBLP:conf/acl/GaoWPLL18} use a learnt world model to generate simulated trajectories.  Different from ours, DDQ uses the world model to generate complete dialogues. As the errors in simulation aggregate, the generated dialogues diverge from the real ones. DDQ aims to improve the sample efficiency of the system agent. But using a large amount of simulated trajectories hampers the performance on the contrary. Observing that, follow-up works focus on improving the quality of simulations. For instance,   D3Q \cite{DBLP:conf/emnlp/SuLGLC18} uses generative adversarial networks (GAN) to minimize the difference between the simulated trajectories and real trajectories. Our method
%is also faced with 
also faces similar challenges, but we handle them in a different way. On one hand, we simulate short trajectories to stop the errors from propagating. On the other hand, we view the simulated trajectories as a forced exploration imposed on the system agent and carefully control the amount of simulated trajectories used for training. By prudently handling the extent of divergence between simulated trajectories and real trajectories, our method trains the system agent better. 

\grace{this chunk should go to related work or removed. chunk begins:}
Previous works on model-based dialogue systems \cite{DBLP:conf/acl/GaoWPLL18} focus on improving the sample efficiency of RL algorithm. In their works, simulated trajectories function as replacements of real ones. With such an objective, some follow-up works \cite{DBLP:conf/emnlp/SuLGLC18} target at improving the quality of simulations and minimizing the discrepancy between these two types of trajectories. \grace{Chunk ends}

\grace{this paragraph is fine. But thinking about combine it with the first paragraph. Or maybe you don need first paragraph? I dont know. The first paragraph was not in good shape so I could not tell what it is for.} 
In our work, instead of generating replacement for real trajectories, we consider simulated experiences as boosters for the training of system agent. Rather than substituting the real trajectories, our method generates simulated trajectories stem from trajectories from real human users, probing different outcomes of the same dialogue. The simulated experiences give the system agent another push to  explore more effectively in the trajectory space \grace{what is trajectory space? Do you need to define it mathematically? Think about it. It might not be a bad idea to define a trajectory mathematically}. 


Model-based approaches have also been studied in the context of other applications. \citeauthor{DBLP:conf/nips/ChuaCML18} proposed probabilistic ensemble trajectory sampling (PETS) and applied it in robotics tasks. PETS learns an ensemble of probabilistic dynamics model for a continuous action space, and uses that ensemble when planning. Apart from the difference in applications, our method works in a discrete action space. Instead of planning before taking every action, our method generates simulated trajectories and uses them for training.    A follow-up work by \citeauthor{DBLP:conf/nips/JannerFZL19} shows that theoretically simulated trajectories can guarantee the monotonic improvement of the policy if the simulation is conducted properly. They propose to begin the simulation by sampling from the state distribution of the previous policy.   While their method only uses simulated trajectories to  update the policy, our method uses both the simulated trajectories and the real trajectories. 

The environment of a task-oriented dialogue system consists of two parts, one is the user, while the other is the database. The system agent converses with the user, and queries the database to complete the task. Our method specifically models the policy of the user. Multi-agent dialogue policy learning (MADPL) \cite{DBLP:conf/acl/TakanobuLH20} shares a similar idea from this point. They consider the user as another agent and formulate the dialogue as a multi-agent RL problem. While their goal is to obtain the system policy and user simulator simultaneously, our method aims to generate diverse training trajectories for the system agent. 

% GDPL \cite{DBLP:conf/emnlp/TakanobuZH19}

% PETS \cite{DBLP:conf/nips/ChuaCML18}, MBPO \cite{DBLP:conf/nips/JannerFZL19}


==> setup.tex <==
\section{Problem Setup}

% \grace{define what is a dialogue, what is the agent to learn eventually (optimization function etc); in MBRL, what is the input/output of the model learning, what is the input/output of the policy learning.}  

% \grace{I am thinking to call 'agent' instead of 'system'. It saves words. okay? and it should apply to entire document. also, database changes to knowledge base (two words). } 

% \grace{Here I temperately put a list of symbols used in the paper. Please update it so that everyone knows how to edit at different places. Our goal is to be consistent within the paper. One concept has only 1 unique name and symbol.\\
% User model: $M$ it can be both base or diversified.  \\
% Base User Model: $M_0$ (I prefer it to be $M_{u}$; what do you think?)\\
% Diversified user model with parameter: $M_{\phi_i}$ \\
% Trajectory: $\tau$ \\
% transition model: $P$ \\
% Ensemble (DUME): D = \{$M$\} \\
% Connecting point: $p$ \\
% horizon: $H$ (not $T$ right? because I saw some $T$) \\
% tuple: $\mathscr{T}_k$\\
% } 
% \zhiwen{$T$ is the length of a base trajectory. It varies in different dialogues. $H$ is the length for a simulation. It is fixed for all dialogues.} \grace{do T and H ever appear in one sentence or one formula, when the branching happens and runs for H steps?}

% A task-oriented dialogue is an interactive process between a user and a dialogue agent, both having access to a knowledge base. The dialogue begins when the user initiates it with a goal in mind and ends when both parties say ``good-bye" or the user abandons the conversation. As the dialogue unfolds, the user can  {\it make requests} for information that she did not know at the beginning of the task. 
% For instance, she may ask the phone number by $phone\_number=?$ when booking restaurant seats. The user can also {\it impose constraints} that restricts the task. For example, the user may set $time=weekend$ in the goal if she only wants to go to movie theaters on weekends. \grace{add the math definitions, e.g. $A$, for dialogue acts here.} 


% \begin{table*}[t]
%     \centering
%     \begin{tabular}{lclll}
%         &{\bf Symbol} & {\bf Meaning} & {\bf Definition} & \makecell[l]{ \textbf{Examples}}\\
%     \midrule
%     Simulator &  $G$ & \makecell[l]{The task goal of\\ the dialogue.} & \makecell[l]{The task goal of dialogue includes 1) cons-\\traints and 2) requests from the user} & \makecell[l]{$1)hotel\ name=Leverton\ House$\\$2)hotel\ address=?$\\$hotel\ phone=?\ hotel \ type=?$} \\   
%             \cline{2-5}
%     &     $s^u_t$ & \makecell[l]{The state of the\\ user at time $t$} & \makecell[l]{The user state includes 1) historical dialogue\\ acts of the agent, 2) dialogue task goal. } & \makecell[l]{$1)[inform\ hotel\ area]$ \\ 2) same as $G$} \\
%          \cline{2-5}
%      &    $a^u_t$ & \makecell[l]{The action of the\\ user at time $t$} & \makecell[l]{Each agent action is a subset of user dialogue\\ acts $A^u$. The user may  perform \\ multiple  dialogue acts at a time step.} & \makecell[l]{$[request\ hotel\ address,$\\$request\ hotel\ phone,$\\$request\ hotel\ type]$}\\
%          \hline
         
%       Agent & $s^s_t$ & \makecell[l]{The state of the\\ conversational \\agent at time $t$} & \makecell[l]{The agent state is a compound that includes:\\ 1) historical dialogue acts of the user, \\2) historical dialogue acts of the agent,\\ 3) dialogue task goal,\\ 4) database querying results.} & \makecell[l]{$1)[inform\ hotel\ name, request\ $\\$hotel\ address,request\ hotel\ phone,$\\$request\ hotel\ type]; 2) [inform\ $\\$hotel\ area];$ 3) same as G;\\ 4) 1 result matches user's constraints}\\
%          \cline{2-5}
%      &    $a^s_t$& \makecell[l]{The action of the \\conversational \\agent at time $t$} & \makecell[l]{Each agent action is a subset of system dialogue\\ acts $A^s$. The agent may perform\\ multiple dialogue acts at a time step.} & \makecell[l]{$[confirm\ hotel\ book]$}\\
%         \cline{2-5}
%       &   $r_t$ &  \makecell[l]{The reward for the \\conversational \\agent at time $t$} & \makecell[l]{ The agent receives $-1$ for every step it takes. At\\ the end of the dialogue, the agent receives $T$ \\ as reward if the dialogue task is completed, \\otherwise $-T$, where $T$ is the length of a dialogue.} & \makecell[l]{$r_t=-1$ since the dialogue has not \\ended yet.}\\
%          \hline
     
%     \makecell{Interaction\\ Tuple}  & $\mathscr{T}_t$ & \makecell[l]{The state-action-re-\\-ward tuple at time $t$} & $\mathscr{T}_t=(s^s_t, a^s_t, r_t, s^u_t, a^u_t)$ & $\mathscr{T}_1 = (s^s_1, a^s_1, r_1, s^u_1, a^u_1)$\\
         
%          \hline
%     \makecell{Trajectory\\  segment} & $\tau_i^{j}$ & \makecell[l]{A sequence of \\interaction tuples starting \\from time step $i$  \\ to time step $j$} & $\tau_i^j  = [\mathscr{T}_i, \mathscr{T}_{i+1}, ... , \mathscr{T}_{j}]$ & $\tau_2^5  = [\mathscr{T}_2, \mathscr{T}_3, \mathscr{T}_4, \mathscr{T}_{5}]$\\
         
%          \bottomrule
%     \end{tabular}
%     \caption{Symbol Definitions}
%     \label{tab:symbol_defn} %\grace{zhiwen, can you add concrete dialogue examples for each row? Better to use example utterance from the running example in Introduction. Thanks}
%     % \grace{I don't think you need two tables (Tables 1 and 2). That will just confuse users. Because you are talking about the same thing, not on two things. If space is an issue, adjust the spacing of each cell or font size. But splitting into two tables would be logically wrong. The rule of thumb is, you should not unnecessarily increase the mental workload (or eye use) of your reader's.}
%     % \grace{Too long as a table title. Be concise. Like a movie's title.} 
% \end{table*}  








% \grace{order of the following paragraphs are weird. The logical order, or the order that most lay-persons would expect to read, is from general to specific. It should be a top-down order. It might not be what you thought the order is for your application. However, your reader is a general audience, not someone working on dialogue acts. For things about RL, people also expect the order of agents --> state  --> action --> reward --> transition --> goal. I suggest: Conversational Search (the task) --> simulator (one of the agents) --> your agent (the other agent)  --> state --> action (aka dialogue act) --> reward  --> tuple  --> trajectory --> goal. If your internal content for each block do not follow this order, please try to edit them inside each block. The dependency would be changed. Because the later concepts will need to built on top of early writing. However, the current order is not following a reader's expectation. Must change. Stuff that conflicting with this order should be trimmed or move to a suitable place in other parts of the article. } 

% \zhiwen{I introduced dialogue acts before states. Because the definition of states also depends on the dialogue acts}

% \hfill

% \grace{1) I don't care. And the readers won't care. We just feel weird. You need to remove the dependency (and this should be more complicated than just cut and paste) or move dialogue act inside state so that dialogue act first appear within state.  2) Things before states, actions, cannot use them. Because they have not been introduced. You need to move those uses of them that belong to "conversational search", "simulator", and "CA" to later places, e.g. within states, actions etc. Rule of thumb -- things cannot be used before they are introduced; and things need to appear based on an order a lay-person can imagine. Don't surprised them unnecessarily. These things are ALL cosmetic. And should be easy to fix. So, a lay-person will judge you based on these things. If you do not obey these rules, you are doomed. 3) So things before your first formal introduction of states, actions, etc will need to be general, vivid, and like a prelude for states, actions, etc. 4) you need to be very careful about this. I think it is indeed about a very difficult and important topic in writing -- organizing a logical outline, trimming, and WHERE to say what. If you do this inappropriately, which I believe it is now, your article looks like a person with a big and ugly cluster of tumor in some parts of his body. An article should have a neat, orderly, and healthy structure.} 

% \hfill

% \grace{And I found that you need to pay more attention to the details. 1) For instance, You cannot have broken underscores between words (e.g. hotel address). 2) It is also not good to have underscores in a name, because they are supposed to be text, no longer your programming code or parameter name. It is different. You need to make sure they look like normal English. 3) In the related work section, thank you for adding the KG-QA section, I like it. However, you forgot to add those new citations into the paragraph above it when they are supposed to be cited at the first time. 4) In the overview paragraph, it is important to cite roughly equal amount of papers for each category. Basically, we are writing an article that is supposed to be an art piece -- so it will need balance in almost every aspect to have aesthetic value. Please help so. thanks.}

{\bf Task-oriented Dialogue Systems} study the interactive process between a user and a dialogue agent while they communicate to accomplish a task. The user initiates the dialogue with a task goal in mind. A task goal can include {\it constraints} and {\it requests}. Constraints are requirements from the user personally and requests are information the user needs but does yet know when the dialogue starts. The goal of a dialogue may span across multiple domains. % E.g., a user wants to book tickets of a movie to be played on weekend but does not know the theater's phone number. Here the constraint is $time=weekend$ and request is $phone\_number=?$. 
In the example in the introduction, the user wants the address of a hotel named Leverton House and also wants to book a train ticket from Peterborough to Cambridge. In this case, the goal of this user involves two domains, \textit{hotel} and \textit{train}. The constraints include $hotel \ name=Leverton\ House$, $train\ departure=Peterborough$, and, $train\ destination=Cambridge$. The requests are $hotel\ address=?$ and $train\ ID=?$. 
A dialogue ends when both parties say ``good-bye" or the user abandons it.  

\hfill

\noindent {\bf Simulators.} As a dialogue unfolds, the user chooses proper actions to either {\it make requests} or  {\it impose  constraints}. In our paper, a user model is equivalent to environment model because the knowledge base is static and no need to learn. We use $s^u_t, a^u_t$  to denote the state and action of a user model at time step $t$. The model learns  a mapping from $s^u_t$ to $a^u_t$ to describe patterns and behaviours from human users, and works as a simulator to provide feedback to and converse with the dialogue agent. 
A user model learns the pattern and behavior from human users and works as a simulator to provide feedback and converse with the dialogue agent. We denote the simulator that is parameterized by $\phi_i$ as $M_{\phi_i}$. A special case is the {\bf expert simulator} $M_0$. It is powered by rules handcrafted by domain experts. 

 %\grace{Grace--change here}\grace{add how U will be used differently for MF and for MB. } In both model-free and model-based settings, $M_0$ is treated as part of the environment. 

%A diversified user model $M$ has the same available dialogue acts ($A^u$) as the base simulator $M_0$. 


\hfill


\noindent {\bf Dialogue Agent} is the policy learner. It is expected to check up the knowledge base, reply the user with relevant information, and make transactions following the user's constraints. We use $s^s_t, a^s_t$ to denote the state and action of the dialogue agent at $t$. The agent also receives reward signal $r_t$ as immediate feedback for its action at time $t$. State transition function $P$ tells its next state which is dependent on the current state and actions from both the user and the agent: $s^s_{t+1} = P(s^s_t, a^s_t, a^u_t)$. The agent learns its policy $\pi$ from a set of dialogue trajectories $\{\tau_*\}$. It aims to maximize the expected cumulative rewards $\mathbb{E}_{\pi} [\sum_t r_t]$ that can be obtained in a dialogue. 

\hfill


\noindent {\bf State} represents the agent's or the user's awareness of the conversation status. To better describe the conversation process, we abstract utterances into {\bf dialogue acts} to illustrate their functions in the context of the conversation. For instance, the question, ``Would you like to go ahead and book it'', conveys a single dialogue act( $book\ hotel\  confirm$), showing the system confirms the booking information with the user. A single utterance may carry multiple dialogue acts. For example, the sentence, ``I would also like to book a train from Peterborough to Cambridge arriving at 15:15 on Sunday'', encodes three dialogue acts: the departure station ($inform\ train\ departure$), destination station ($inform\ train\  destination$), and arrival time ($inform\ train\ arrive\ By$). The system and the  user may have different set of available dialogue acts. We denote them as $A^s$ and $A^u$, respectively.


The states of both the user and the agent are compounds that include different types of information. The agent state $s^s_t$ consists of 1) the task goal of the user, 2) historical dialogue acts of both the agent and the user, 3) database querying results based on the identified user's constraints. The user state ($s^u_t$) includes 1) the task goal of the user and 2) the historical dialogue acts of the agent.  The formulations depict the conversation from different perspectives and provide sufficient information for decision-making. 



\hfill

\noindent {\bf Actions} are defined as the dialogue acts that the user or the system picks at each turn. The number of dialogue acts picked by the user or the system varies turn by turn. Mathematically, the system action $a^s_t$ is a subset of $A^s$, and the user action $a^u_t$ is a subset of $A^u$. We represent $a^s_t$ and $a^u_t$ as lists of indicator variables in the length of $|A^s|$ or $|A^u|$. 

There are multiple different ways to transform dialogue acts into natural language utterances. But such generation process is not the focus of our work. In this paper, we use pre-defined templates to generate natural language utterances from the selected dialogue acts. 



\hfill

\noindent {\bf Reward} We design the reward function to motivate the agent to complete tasks with fewer times of interactions. The agent receives $T$ as a reward if it completes the task, otherwise $-T$, where $T$ is the number of interactions in a conversation. Before reaching the end of a conversation, the agent receives a reward of $-1$ for every step it takes. 


 
% \hfill

% \grace{Zhiwen, more concrete examples are needed in the paragraphs you added here. Better to use example utterance from the running example in Introduction.}



% \hfill

% \noindent {\bf Actions} An agent action or a user action may contain multiple dialogue acts. A dialogue act is an atom operation that the agent takes to interact with the user and complete the task. An example dialogue act is `booking-request-time' \grace{this example is good but too brief. We need vivid examples.}, which denotes that the agent requests the time from the user to complete a booking. The user or the agent may perform multiple dialogue acts at a single step. The dialogue acts available to the user and the agent are different. Mathematically, the agent action $a^s_t$ is a subset of $A^s$, and the user action $a^u_t$ is a subset of $A^u$, where $A^s$ and $A^u$ are the sets of dialogue acts for the agent and the user, respectively. 





%In this paper, we propose to diversify the training trajectories $\{\tau_i\}$ with trainable user models $M$, to best improve the effectiveness of the dialogue agent's policy. 

%In our context, the world to a dialogue agent include both a knowledge base and a user simulator. Since the knowledge base is not dynamically changing, our world modeling focuses only on user modeling. 

% \grace{how to use the above notations to define the problem of model learning? and how to denote real trajectories and simulated trajectories? how to define the extension function? how to show an ensemble of user models? trajectories? how to measure the diversity of a group of trajectories?}

\hfill



\noindent {\bf Interaction Tuple $\mathscr{T}$} is the state-action-reward tuple generated when the agent interacts with a user model. At the $t^{th}$ dialogue turn, the $t^{th}$ interaction tuple is
 $\mathscr{T}_t = (s^s_t, a^s_t, r_t, s^u_t, a^u_t)$. 
 
 %\grace{why you need to start from $k$? Can you define it as --- $\tau  = [\mathscr{T}_1, ...,  \mathscr{T}_{k}, ... ,\mathscr{T}_{T}]$? Or just $\tau  = [\mathscr{T}_1, ...,  \mathscr{T}_{t}, ... ,\mathscr{T}_{T}]$? }  \zhiwen{No, a branching trajectory would start halfway}

\hfill


% \grace{1) For trajectory segment, it is important that you introduce both starting and ending points in its formulation. I remember this is where I had a lot of confusion. Now I think you were right they should have beginning and ending -- two inputs points. However, what you confused me before was the English -- trajectory isn't segment. I now understand what you meant was ``segment" or ``trajectory segment". I suggest to use the wording ``trajectory segment". Then you must edit anywhere it appears to match this idea of two inputs. 2) For ``trajectory", it should be the collection or ordered set of trajectory segments. And you should show their differences and their conceptual connection -- one is the other's hyponym parent conceptually. And this should be shown ivisibility in your writing and presentation. Remember, good designs are invisible. I urge you to read and edit and read and edit ... until you feel comfortable, with no hiccups when you read it. For every hiccups in the draft, you must change it. Fix it. Make it smooth.}

\noindent {\bf Trajectory $\tau_k^{k+h}$} 
is a sequence of interaction tuples generated when the agent interacts with $M_0$ or $M_{\phi_i}$, starting from time step $k$ and lasting for $h$ steps: $\tau_k  = [\mathscr{T}_k, \mathscr{T}_{k+1}, ... , \mathscr{T}_{k+h}]$, 
where $\mathscr{T}_t$ is the $t^{th}$ interaction tuple.  Decided by state transition $P$, latter interaction tuples in $\tau$ depend on the earlier tuples. 

\begin{itemize}
    \item An {\bf expert trajectory} is a trajectory that records the interaction between the agent and the expert simulator $M_0$.
    \item A {\bf full trajectory}, $\tau_0^T$ , is a trajectory running from $0$ to $T$, where $T$ is the dialogue length and marks the end of a conversation. 
\end{itemize}

\begin{comment}
\begin{itemize}
   \item A {\bf trajectory segment $\tau_x^y$} is a trajectory that records the interaction between $M_0$ and the agent. It usually starts from the dialogue's beginning, $k=0$.  An {\bf expert trajectory segment $\tau_0$} is a trajectory that records the interaction between $M_0$ and the agent. It usually starts from the dialogue's beginning, $k=0$.

  \item A {\bf full  trajectory $\tau_0^{full}$=$[\mathscr{T}_0 ..., \mathscr{T}_{T}]$} is a base trajectory running from $0$ to $T$, where $T$ is the dialogue length and marks the end of the dialogue.  A {\bf full expert trajectory $\tau_0^{full}$=$[\mathscr{T}_0 ..., \mathscr{T}_{T}]$} is a base trajectory running from $0$ to $T$, where $T$ is the dialogue length and marks the end of the dialogue.
  
\end{itemize}
\end{comment}

  
\noindent The {\bf Optimization Goal} is to generate diverse trajectories by interacting with trainable user models ($M_{\phi_i}$) to maximize the cumulative reward when interacting with the expert simulator ($M_0$).


% The user and the knowledge base form the world that the agent interact with. Since content of the knowledge base is static, our world modeling focuses only on user modeling. The user model is defined as follows. We use $s^u_t, a^u_t$  to denote the state and action of the user at time step $t$. The learning of this user MDP is done by imitation learning.  Additionally, we use $d_t$ to mark $t$ is the end of the dialogue. 
% \grace{move stuff about user MDP setup in section 3.3 here.} 


% \grace{what is our main task here? dialogue policy learning or trajectory diversification? How to show both problems mathematically here?}
